A Snowmass Whitepaper: Dark Matter Production at Intensity-Frontier Experiments

Dark matter particles can be observably produced at intensity-frontier experiments, and opportunities in the next decade will explore important parameter space motivated by thermal DM models, the dark sector paradigm, and anomalies in data. This whitepaper describes the motivations, detection strategies, prospects and challenges for such searches, as well as synergies and complementarity both within RF6 and across HEP.

==> Big Idea 1/workshopsymbols.tex <==
%%%%   Standard symbols for use in Snowmass Working Group Proceedings%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  basic formatting macros:%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%   text mode macros

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

\def\Acknowledgements{\bigskip  \bigskip \begin{center} \begin{large}
             \bf ACKNOWLEDGEMENTS \end{large}\end{center}}


%  equation display macros

\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

%%  reference to an equation number:

\def\leqn#1{(\ref{#1})}

%%  sizing and bars

\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}

\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

\def\subscr#1{{\mbox{\scriptsize #1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values: 

\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% relation symbols

\def\lsim{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\gsim{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}

\def\Im{{\rm Im}}
\def\Re{{\rm Re}}
\def\tr{{ \rm tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}
\def\H{{\cal H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{\not{\hbox{\kern-4pt $E$}}_T}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\GUT{{\mbox{\scriptsize GUT}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\gw{\Gamma_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_H}
\def\gh{\Gamma_H}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\MSB{{\bar{M \kern -2pt S}}}
\def\msb{{\bar{\scriptsize M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\drb{{\bar{\scriptsize D \kern -1pt R}}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}
\def\Kzero{K^0}
\def\Kzerobar{{\bar K}^0}
\def\Dzero{D^0}
\def\Dzerobar{{\bar D}^0}
\def\Bzero{B^0}
\def\Bzerobar{{\bar B}^0}


%%%%%%%%%%%%   units for math mode  %%%%%%%%%%%%%%%%%%%%%%%%%

\def\ifb{{\rm fb}^{-1}}
\def\eV{{\rm eV}}
\def\keV{{\rm keV}}
\def\MeV{{\rm MeV}}
\def\GeV{{\rm GeV}}
\def\TeV{{\rm TeV}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}



%%%%%%%%%%  common journal names   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\newcommand\aj{{Astronomical Journal}}%
%\newcommand\araa{{Annual Review of Astron and Astrophys}}%
% \newcommand\apj{{Astrophysical Journal}}%
%\newcommand\apjl{{Astrophysical Journal, Letters}}%
%\newcommand\apjs{{ApJS}}%
%% Astrophysical Journal, Supplement
%\newcommand\ao{{Appl.~Opt.}}%
%% Applied Optics
%\newcommand\apss{{Ap\&SS}}%
%% Astrophysics and Space Science
%\newcommand\aap{{Astronomy and Astrophysics}}%
%\newcommand\aapr{{A\&A~Rev.}}%
%% Astronomy and Astrophysics Reviews
%\newcommand\aaps{{A\&AS}}%
%% Astronomy and Astrophysics, Supplement
%\newcommand\azh{{AZh}}%
%% Astronomicheskii Zhurnal
%\newcommand\baas{{BAAS}}%
%% Bulletin of the AAS
%\newcommand\jrasc{{JRASC}}%
%% Journal of the RAS of Canada
%\newcommand\memras{{MmRAS}}%
%% Memoirs of the RAS
%\newcommand\mnras{{Monthly Notices of the Royal Astronomical Society}}%
%\newcommand\pra{{Phys.~Rev.~A}}%
%% Physical Review A: General Physics
%\newcommand\prb{{Phys.~Rev.~B}}%
%% Physical Review B: Solid State
%\newcommand\prc{{Phys.~Rev.~C}}%
%% Physical Review C
%\newcommand\prd{{Physics~Review~D}}%
%% Physical Review D
%\newcommand\pre{{Phys.~Rev.~E}}%
%% Physical Review E
%\newcommand\prl{{Phys.~Rev.~Lett.}}%
%% Physical Review Letters
%\newcommand\pasp{{Publications of the ASP}}%
%\newcommand\pasj{{PASJ}}%
%% Publications of the ASJ
%\newcommand\qjras{{QJRAS}}%
%% Quarterly Journal of the RAS
%\newcommand\jcap{{JCAP}}%
%\newcommand\skytel{{S\&T}}%
%% Sky and Telescope
%\newcommand\solphys{{Sol.~Phys.}}%
%% Solar Physics
%\newcommand\sovast{{Soviet~Ast.}}%
%% Soviet Astronomy
%\newcommand\ssr{{Space~Sci.~Rev.}}%
%% Space Science Reviews
%\newcommand\zap{{ZAp}}%
%% Zeitschrift fuer Astrophysik
%\newcommand\nat{{Nature}}%
%\newcommand\iaucirc{{IAU~Circ.}}%
%% IAU Cirulars
%\newcommand\aplett{{Astrophys.~Lett.}}%
%% Astrophysics Letters
%\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}%
%% Astrophysics Space Physics Research
%\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}%
%% Bulletin Astronomical Institute of the Netherlands
%\newcommand\fcp{{Fund.~Cosmic~Phys.}}%
%% Fundamental Cosmic Physics
%\newcommand\gca{{Geochim.~Cosmochim.~Acta}}%
%% Geochimica Cosmochimica Acta
%\newcommand\grl{{Geophys.~Res.~Lett.}}%
%% Geophysics Research Letters
%\newcommand\jcp{{J.~Chem.~Phys.}}%
%% Journal of Chemical Physics
%\newcommand\jgr{{J.~Geophys.~Res.}}%
%% Journal of Geophysics Research
%\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}%
%% Journal of Quantitative Spectroscopy and Radiative Transfer
%\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}%
%% Mem. Societa Astronomica Italiana
%\newcommand\nphysa{{Nucl.~Phys.~A}}%
%% Nuclear Physics A
%\newcommand\physrep{{Phys.~Rep.}}%
%% Physics Reports
%\newcommand\physscr{{Phys.~Scr}}%
%% Physica Scripta
%\newcommand\planss{{Planet.~Space~Sci.}}%
%% Planetary Space Science
%\newcommand\procspie{{Proc.~SPIE}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
